Ultrasound Phase Aberrated Point Spread Function Estimation with Convolutional Neural Network: Simulation Study

Ultrasound imaging systems rely on accurate point spread function (PSF) estimation to support advanced image quality enhancement techniques such as deconvolution and speckle reduction. Phase aberration, caused by sound speed inhomogeneity within biological tissue, is inevitable in ultrasound imaging. It distorts the PSF by increasing sidelobe level and introducing asymmetric amplitude, making PSF estimation under phase aberration highly challenging. In this work, we propose a deep learning framework for estimating phase-aberrated PSFs using U-Net and complex U-Net architectures, operating on RF and complex k-space data, respectively, with the latter demonstrating superior performance. Synthetic phase aberration data, generated using the near-field phase screen model, is employed to train the networks. We evaluate various loss functions and find that log-compressed B-mode perceptual loss achieves the best performance, accurately predicting both the mainlobe and near sidelobe regions of the PSF. Simulation results validate the effectiveness of our approach in estimating PSFs under varying levels of phase aberration.

==> submission/01-Related_Work.tex <==
\section{Related Work}

\textbf{Speckle Reduction.} Speckle reduction is the most common image enhancement technique used in ultrasound imaging. The goal is to completely or conservatively remove speckle noises so that images own better visual quality. Many efforts have been put into speckle reduction algorithms \cite{OBNLM,SRAD,SR_BM3D,SR_wavelet,WRNLM}. Speckle reduction algorithms preserve the sharpness of image borders by limiting speckle noise suppression along edges and borders \cite{review_us_postprocessing}, whereas our image sharpening technique actively increases the border sharpness. In the discussion section, we show that our image sharpening technique could be cascaded to speckle reduction algorithms and the image quality could be further improved.

\textbf{Gradient Operators.} Canny edge detector \cite{canny} is a popular edge detection method based on image gradients. Some adopted the Canny detector to ultrasound images by using different blurring methods \cite{canny_adjusted,canny_SRAD,canny_multiplicate_gradient} before gradient calculation. These edge detection methods aim for a single response of an edge and generate a binarized edge image. However, in image sharpening, we need a feature mask that is with thick edges or borders and not necessarily binary. Furthermore, these methods mainly rely on the speckle-free images and thus removal of speckle noises is required in advance to gradient calculation. In this work, we directly detect the features with the presence of speckles. This leads to a more generalizable algorithm with fewer parameters.

\textbf{Information Theory Based Feature Detection.}
Information theory based feature detection uses a sliding window with two sub-windows and models the two speckle distributions in the sub-windows into Rayleigh or FT distributions \cite{info_edge_detection,info_ultrasound_feature}. Then, the Jensen-Shannon (JS) divergence is computed between the two distributions and high JS divergence indicates high edge response. Such approaches directly detect features with the presence of speckles. However, the detected features suffer spatial displacements from their original locations, i.e., localization errors. Though this may not be an issue for feature detection or edge detection \cite{edge_similarity_metric}, it will cause sharpening of the images in inaccurate locations and generate sharpening artifacts. This is a common issue of comparison-based feature detection that uses sub-windows. In this work, we only use one sliding window for local statistics estimation without the need for sub-windows.

\textbf{Local Statistics Spread for Feature Detection.} The local statistics spread approaches use a sliding window and measure the spread (dispersion) in each windowed region to detect features. Generally, a larger spread indicates the window is in feature regions whereas a lower spread indicates the homogeneous background regions. Fully-developed ultrasound speckles statistically follow Rayleigh distribution in envelope data and have a constant variance characteristic after log compression \cite{speckle_statistics,speckle_model}. Wang and Liu utilize the constant variance characteristic and use the local histogram range image (LHRI) to detect features \cite{LHRI}, and similarly, Singh \textit{et al.} other local statistical measurement methods \cite{multifractal}. Note that in this work, to improve computational speed, we simply use the local variance for spread measurement, which does not involve time-consuming median or histogram calculation. Furthermore, we address the window size trade-off issue by using a multi-window detection framework that can increase the robustness of feature detection.

==> submission/Keywords.tex <==
Point spread function (PSF) estimation, Phase aberration, Deep learning, Ultrasound imaging.
